Establishing Cyber Resilience in Embedded Systems for Securing Next-Generation Critical Infrastructure

The mass integration and deployment of intelligent technologies within critical commercial, industrial and public environments have a significant impact on business operations and society as a whole. Though integration of these critical intelligent technologies pose serious embedded security challenges for technology manufacturers which are required to be systematically approached, in-line with international security regulations. This paper establish security foundation for such intelligent technologies by deriving embedded security requirements to realise the core security functions laid out by international security authorities, and proposing microarchitectural characteristics to establish cyber resilience in embedded systems. To bridge the research gap between embedded and operational security domains, a detailed review of existing embedded security methods, microarchitectures and design practises is presented. The existing embedded security methods have been found ad-hoc, passive and strongly rely on building and maintaining trust. To the best of our knowledge to date, no existing embedded security microarchitecture or defence mechanism provides continuity of data stream or security once trust has broken. This functionality is critical for embedded technologies deployed in critical infrastructure to enhance and maintain security, and to gain evidence of the security breach to effectively evaluate, improve and deploy active response and mitigation strategies. To this end, the paper proposes three microarchitectural characteristics that shall be designed and integrated into embedded architectures to establish, maintain and improve cyber resilience in embedded systems for next-generation critical infrastructure.

==> AdaptiveSoC/AdaptiveSoC.tex <==
\section{Adaptive System-on-Chip Platform}

Emerging embedded computing architectures such as \textit{Multiprocessing System-on-chip} (MPSoC) provide heterogeneity, scalability, high performance compute and connectivity that can used to realise diverse intelligent applications.
%%
%% Overview of FPGA technology, benefits and oppurtunities to harness security features
%%
Field programmable gate array (FPGA) is a proven reconfigurable technology that provides glue-logic to develop and implement dedicated hardware logic, accelerate computationally intensive applications, essential to deliver the performance and power demands of next-generation intelligent systems. The availability of FPGA MPSoC architectures have extended this appeal, enabling tight integration of hardware and software co-design, allowing customisations after deployment. Significant research work has been published, demonstrating advanced and diverse application use cases can be implemented using FPGA technology [REFS]. The high parallelism available in these MPSoCs is becoming a key enabler platform to support and implement artificial intelligence and machine learning solutions [XILINX INFERENCE]. This evolving trend for has seen FPGA manufacturers integrate various security, safety and power management mechanisms into their newer MPSoC architectures. These FPGA MPSoC architecture offers hardware components for building a security foundation, based on the principles of information assurance, trust and security~\cite{Ray2018}. It includes dividing a system into multiple subsystems, which allows partitioning, isolation and segregation of system resources. 

Unfortunately, vast majority of the embedded devices have been designed, developed and deployed without taking security into account [REF]. There are multiple applications that can be executed simultaneously where some of them execute tasks that require the integration to the cloud [REF]. This sharing of computational and communication resources bring benefits and opportunities and at the same time presents security risks. The increasing complexity of embedded device and hyper-sharing of the hardware resources of MPSoC is becoming a serious security concern as found vulnerable and compromised as reported by the research community [REFS].

%\begin{itemize}
%\item Though, these micro-architectural defense mechanisms has been designed to counter specific vulnerabilities:
%	\begin{itemize}
%	\item Memory protection extension (Memory overflow)
%	\item Pointer authentication (Pointer integrity)
%	\item Control-flow integrity (Code re-use)
%	\item Logical Isolation/Virtualisation (side-channel Information leakage)
%	\item Root-of-Trust                                   
%	\item Chain-of-Trust (Downgrade attack)
%	\end{itemize}
%
%\item There is a clear need for a multi-layered security platform architecture which is flexible and configurable security components which shall be incorporated during architecture design.
%\item Platform Security Design Criteria (Some points are extended from [REF])
%
%	\begin{itemize}
%	\item The security components shall have minimum impact on area and performance of the platform. (By allocating security related tasks to RPU, the performance overhead is minimal on the APU.)
%	\item The platform security component/processor should be independent, physically isolated than computation unit and have the highest priority. (Physical isolation of the platform security processor would significantly reduce the likelihood of information leakage.)
%	\item These multi-layered defense mechanisms supported by the platform shall complement the existing on-chip security mechanisms.
%	\item The platform security architecture shall provide pro-active runtime (dynamic) monitoring by complementing static trusted computing mechanisms such as Secure Boot, Secure Update. (It will provide means to realise active trusted computing state within the platform providing both static (boot-up) and dynamic (pro-active) root-of-trust.)		
%	\end{itemize}
%\end{itemize}

==> Background/Background.tex <==



==> NIST/SoC.tex <==
\section{FPGA MPSoC: A flexible embedded security platform}
\label{sec:MPSoC}
%%
%%
\begin{table*}[!t]
\centering
\scriptsize
\caption{Comparison of on-chip security features supported by leading FPGA MPSoCs~\cite{XilinxFIPS2016},~\cite{XilinxUltraScale2017}.}
\label{tab:mpsoc-comparison}
\begin{tabular}{|l||c|c||c|c|}
\hline
\textbf{FPGA Vendors} & \multicolumn{2}{c||}{\textbf{Xilinx}} & \multicolumn{2}{c|}{\textbf{Intel (Altera)}} \\
\hline
%\hline
\textbf{MPSoC Chips} & \textbf{Zynq-7000} & \textbf{Zynq UltraScale+} & \textbf{Arria 10} & \textbf{Stratix 10} \\
 (technology) & (28nm) & (16nm) & (20nm) & (14nm) \\
\hline
\hline
\rowcolor{AliceBlue} Symmetric Encryption & AES-CBC 256 & AES-GCM 256 & AES-CTR 256 & AES-GCM 256 \\
\rowcolor{AliceBlue} Asymmetric Encryption & RSA & RSA-4096 & RSA, ECC & RSA, ECC \\
\hline
%\hline
\rowcolor{BlanchedAlmond} Integrity check & SHA-256 & SHA-3/384 & SHA-256/384 ECDSA & HMAC-SHA-256, SHA-256/384, ECDSA\\
%\rowcolor{BlanchedAlmond} &  &  &  &  SHA-256/384, ECDSA\\
\hline
%\hline
\rowcolor{Beige} Key Storage & BBRAM, eFUSE & BBRAM, eFUSE, PUF KEK & BBRAM, eFUSE & BBRAM, eFUSE \\
%\hline
\rowcolor{Beige} Hardware root-of-trust & No & PUF (Ring Oscillator) & No & PUF (SRAM pattern) \\
%\hline
\rowcolor{Beige} Unique Identifier (OEM) & eFUSE & eFUSE(plain, obfuscated, and encrypted) & eFUSE & eFUSE \\
%\hline
\rowcolor{Beige} Key Agility (update) & No & Yes & No & Yes \\
\hline
%User access to Crypto & No & Yes & No & Yes \\
%\hline
\rowcolor{LightYellow} Chain-of-Trust & Secure boot, & Secure boot, & - & Secure boot,  \\
\rowcolor{LightYellow} &  ARM TrustZone &  ARM TrustZone    &   &  ARM TrustZone \\
\hline
%\hline
\rowcolor{LightGreen} Side-channel protection & No & DPA resistant & Yes & Yes \\
%\hline
\rowcolor{LightGreen} Anti-tamper detection & No & Yes & No & Yes \\
%\hline
\rowcolor{LightGreen} Tamper logging & No & Yes & No & No \\
\hline
%\hline
\rowcolor{MistyRose} Hardened read-back & Yes & Yes & No & Yes \\
%\hline
\rowcolor{MistyRose} Debug Enable/Disable & Yes & Yes & Yes & Yes\\
\hline
\end{tabular}
\end{table*}
%%
%%
%%
%% Provide evidence of its sucess and advancements in MPSoC technology and brief introduction to ARM TrustZone
%%
The increasing demand for embedded security has driven FPGA vendors to integrate multiple levels of security, increased safety, and advanced power management mechanisms into newer generation of FPGA MPSoCs such as Xilinx Zynq UltraScale+ and Intel Stratix 10. These MPSoCs offer improved built-in hardware security features to harness and deploy system-level security by protecting the system assets~\cite{XilinxFIPS2016},~\cite{XilinxUltraScale2017},~\cite{Polian2017}. Table~\ref{tab:mpsoc-comparison} presents a detailed comparison of the on-chip hardware security features supported by market leading MPSoCs from Xilinx and Intel (Altera). They provide hardware components for building a system security foundation, based on the principles of \textit{information assurance}, \textit{trust} and \textit{security}. They allow partitioning of system resources by dividing a system into subsystems and isolating the memory-space of these subsystem. To support flexibility of software-hardware co-design practices, these security services are extended beyond the general purpose multiprocessing cores (ARM Cortex-A) down to the FPGA glue logic, to address system security issues at the application and user level. It facilitates a software controlled and hardware-enforced approach towards system security. The system software could execute as a standalone bare-metal application, real-time operating system, or full fledge rich-operating system (Embedded Linux, PetaLinux etc.) or combination thereof. The ARM TrustZone is an example that virtually segregates the hardware resources into secure and non-secure worlds, inspired by the concept of privileged and unprivileged access, supported by the operating systems~\cite{Winter2008},~\cite{Santos2014}.

==> PolicyEngine/Figs/RelatedWork.tex <==
\section{Related-work}
\label{sec:related-work}
%%
%%
This section will survey security vulnerabilities reported in the open literature on embedded MPSoC architectures and their supported security features.

%%
%% Reported attacks against ARM TrustZone technology
%%
Chen~\etal exploited a lack of proper rollback protection within numerous devices' \textit{secure boot} process, breaching the loading verification process used by ARM's TrustZone technology. An old key was reused to load a malicious application that could run in the secure-world, providing access to device's secret data~\cite{Chen2017}. Jacob~\etal described an attack against the \textit{secure boot} mechanism on FPGA MPSoC, which ensures secure system start-up and building chain-of-trust in embedded devices~\cite{Jacob2017}. This attack allowed modification of boot parameters to load an unauthorised kernel image from a remote server over the network, instead of booting from the verified source. Though, mitigation of these attacks by formulating a well-defined policy for distributing patches and updating configurations to revoke older software versions, across a wide range of devices, is difficult from a practical perspective. Lipp~\etal further attacked the ARM TrustZone security extension using side-channel analysis. By monitoring cache activity in the special area of the Android operating system, they were able to infer and extract details of the last running process~\cite{Lipp2015}. A potential mitigation of cache attacks is deploying separate caches for each virtual context, as introduced in the latest ARM Cortex-M processors.

%%
%% Concept of Hardware firewall using security policies
%%
Cotret~\etal proposed a \textit{hardware firewall} architecture that enforces programmable security policies to protect external and internal traffic in FPGA based multiprocessor architectures, serving as a security bridge between the system resources and the shared system communication bus to monitor control activities. Their proposed work reduces the performance penalty compared to a fully encrypted approach, however it is limited to the detection of attacks and does not provide countermeasures, other than freezing the system communication bus~\cite{Cotret2016}.
%%
%% Security evaluation of FPGA MPSoC and AXI4 specific vulnerabilities
%%
Jacob~\etal presented a detailed study of FPGA MPSoC security mechanisms with the focus on \textit{Hardware Trojans}~\cite{Jacob2017HWTrojan}. They proposed the concept of a light-weight AXI-wrapper as one of the prevention methods, similar to one proposed by~\cite{Cotret2016}, to encapsulate system assets. Following this work, Benhani~\etal presented a security evaluation of the ARM TrustZone technology available on FPGA MPSoC. They presented some possible hardware attack scenarios caused by the presence of \textit{Hardware Trojans} residing within an MPSoC's FPGA logic~\cite{Benhani2017}. They demonstrated the modification of the hardware security attributes (set by ARM TrustZone) and propagation to the host processor by targeting AMBA-AXI4 communication system bus. These \textit{Hardware Trojans} can be introduced during chip manufacturing process or at different stages of the design and development life-cycle. To mitigate these vulnerabilities, they proposed dividing the system into secure and non-secure subsystems. However, this strategy is not viable for systems with mixed criticality~\cite{Tan2016},~\cite{Tan2017}.

%%-----------------------------------------------------------------------------------------------------
%% 
%%-----------------------------------------------------------------------------------------------------
\subsection{Shortcomings of existing security approaches}
\label{subsec:shortcomings}
%%
%%
After reviewing different aspects of security vulnerabilities and state-of-art of secure architectures and their methodologies to protect system's critical assets, there is clear evidence that existing approaches fall short due to:
%%
%%
\begin{itemize}
\item Security architectures rely on building and maintaining a robust \textit{chain-of-trust}. This \textit{chain-of-trust} is based on a nested series of assumptions and as vulnerable as its weakest link which, once broken, compromises the security of the complete system.
%even a single vulnerability can be exploited to break the chain-of-trust leading to compromised system.
\item A lack of security aware design and development practises, leading to the development of inconsistent and vulnerable software applications by the developers.
\item Complex hardware-software co-design and integration practices, giving rise to vulnerabilities in hardware and software protocol stack boundaries, allowing to launch insider and outsider attacks.
\item Lack of availability of independent run-time security mechanisms that can detect, curtail and secure system assets in hardware if the existing system security mechanisms are compromised. It includes systems with compromised \textit{chain-of-trust}.
%
%\item Lack of hardware security standards and protocols which vendors can use to evaluate security of developed hardware and software components before and after integrating them into the system to ensure secure product development life-cycle.
\end{itemize}


==> PolicyEngine/PolicyEngine_Conflict_.tex <==
%%----------------------------------------------------------------------------------%%
%% 					Embedded Policing and Policy approach
%%----------------------------------------------------------------------------------%%
\section{Embedded policing and policy enforcement approach}
\label{sec:policing-approach}
%%
%%
%%
%%
\begin{figure*}[!t]
\centerline{\includegraphics[scale=0.70]{PolicyEngine/Figs/platform}}
\caption{System architecture to implement the proposed policing and policy enforcement approach to harness and enforce defined security policies within FPGA MPSoC platform.}
\label{fig:platform}
\end{figure*}
%%
%%
To approach the identified shortfalls, we propose a policing and policy enforcement approach that shall enhance system security, scalability, provisioning during operational life-cycle by complementing existing security mechanisms available in MPSoC based embedded architectures. This policing approach shall monitor the undergoing communication of system resources and compare it against the expected (secure) behaviour. In case of unexpected behaviour, for example a malicious action from a compromised application or initiated by a \textit{Hardware Trojan} or launching of attack by the adversary, the system can take both the active and passive counter-measures to mitigate the attack and ensure the protection of the system assets. Expected behaviours shall be defined as the system \textit{security policy}, which can be updated at any stage of the device life-cycle. The policing approach, deployed at system communication layer, will be transparent to existing embedded system architectures and security extensions (such as ARM TrustZone) that use the de-facto industry standard ARM AMBA-AXI4 SoC bus communication protocol, along with their software stacks (bare-metal, embedded Linux, RTOS, Hypervisor, device drivers etc.) The proposed policing and policy enforcement system architecture will not only enhance security of the device, but will also improve flexibility to meet dynamic security requirements of next generation embedded architectures, as well as the next-generation of threats.

%%----------------------------------------------------------------------------------%%
%% 			MPSoC based embedded policing platform architecture
%%----------------------------------------------------------------------------------%%
\subsection{Embedded policing platform architecture}
\label{subsec:platform-architecture}
%%
%%
Embedded systems are complex, with system designers and software developers often required to consolidate different functionalities into a single application which usually requires combining of sensitive and non-sensitive data together. Heterogeneous multiprocessor system-on-chip (MPSoC) platforms, composed of multiple processors, hardware IPs, on-chip support of peripheral interfaces and shared memory resources, are a suitable choice to achieve manifold design goals, as this aids adaptability, re-usability, portability and upgradability and accelerates product design, development, testing leading to reduce time-to-market which gives economical benefits to the solution provider. Nevertheless, they offer on-chip hardware security features as previously outlined in Table~\ref{tab:mpsoc-comparison}, to protect the assets and attain security that is critical requirements of next-generation secure embedded systems.

To realise the proposed policing and policy enforcement approach, Fig.~\ref{fig:platform} present a system architecture that uses Xilinx Zynq UltraScale+ MPSoC. This platform has chosen due to availability of on-chip \textit{cryptographic} and \textit{hardware security} features including \textit{Hardware root-of-trust} (HRoT) which previously not available as detailed in Table~\ref{tab:mpsoc-comparison}. However, the proposed embedded policing approach is not limited to the chosen platform and can be integrated to any AMBA-AXI4 compliant ASIC or SoC architecture. It can be adopted into existing and new embedded architectures at any stage of design and development process, to establish or enhance the hardware security into new or existing embedded architectures.

The MPSoC features an on-chip Quad-core ARM Cortex-A53 \textit{Application Processing Unit} (APU) for general purpose computing, and a Dual-core ARM Cortex-R5 \textit{Real-time Processing Unit} (RPU) for deterministic time critical computing. The APU cores can be configured to use for symmetric and asymmetric multiprocessing  and supports multiple software stack configurations to match the diverse computing requirements of the applications. It supports execute of wide range of independent software stacks simultaneously on these APU cores such as bare-metal, unsupervised, supervised and hypervised software applications~\cite{XilinxUltraScale2017}. It has an ARM TrustZone hardware security module that extends and propagates the secure attributes of the software applications down to shared ARM AMBA-AXI4 system-bus. 
%It has achieved by segregating generated data and control transactions into secure and non-secure world, which limits access to the system resources.

In proposed system architecture, it is assumed that \textit{untrusted software stack} executes on APU and can access its connected resources. Moreover, it is assumed that all security related tasks which includes configuration, provisioning and management of the proposed policing components will execute on the RPU and will be treated as a \textit{trusted application}. Since, RPU has a dual 64 KB \textit{tightly-coupled memory} (TCM), that is physically isolated from L1 and L2 cache of the APU. This system security boundary is highlighted in Fig.~\ref{fig:platform}. This physical isolation and segregation between APU and RPU ensures that any \textit{untrusted application} cannot read, write or modify any part of the TCM. This approach could encounter the shortcomings of the security architectures that uses virtualisation. Central to our proposed policing and policy enforcement approach are the following hardware components:
%%
%%
\begin{enumerate}
	\item Security policy engine   (SPE)
	\item AXI4-Bus sanity checker  (SCK)
	\item Security response engine (SRE)
	\item Anti-tamper engine       (ATE)
\end{enumerate}
%%
%%

The SPE and SCK are implemented on FPGA glue logic while, SRE and ATE use the hardware security features of Xilinx Zynq UltraScale+ MPSoC. They allow to:
%%
%%
\begin{itemize}
	\item Monitor system-level communication between master and slave data and memory peripherals, and enforce the defined security policies for each slave.
	\item Check the sanity of system-bus at the interface between host processor and hardware IP's to detect and curtail \textit{insider} and \textit{Hardware Trojans} attack.
	\item Initiate passive or active response against vulnerabilities and attacks caused either by \textit{insider} or \textit{outsider} attacks, and protect system's critical assets.
\end{itemize}
%%
%% 

Each hardware component has an AXI4-Lite interface that RPU uses to configure, program and manage their supported security features. One of the benefits of this approach is silicon manufacturer, third-party vendors and hardware designers could carry independent provisioning of their secure embedded devices by defining resource specific policies during the operational life-cycle of their device~\cite{Jacob2017Provision}. Nevertheless, as the proposed hardware components uses the FPGA glue logic, So they are portable and can be used in versatile embedded hardware architectures to incorporate hardware security.

The AXI4 communication bus establishes a communication between a master and a slave using five separate channels; \textit{address write, write data, write response, address read} and \textit{read data} as detailed in the ARM AMBA-AXI4 protocol specification~\cite{XilinxUltraScale2017},~\cite{ARMAXI2017}. Each channel has a VALID and READY handshake signal that represents the validity of data available on the bus, and indicates that the receiver is ready to receive the data available on the bus respectively. The exchange of data happens when both VALID and READY signals are high.

To incorporate system level security, the AXI4 supports additional control signals~\cite{XilinxUltraScale2017},~\cite{ARMAXI2017}. Both address channels have 3-bit AWPROT and ARPROT signal, the second bit of which is \textit{Non-Secure} (NS)-bit that defines the security attribute of the transactions. 
%These security attributes are initiated either by the host processor, or by the hardware security designer to mark different part of the system either secure or non-secure. 
During system execution, they propagate down to the FPGA glue logic through the system interconnect (AXI4-Interconnect) as shown in Fig.~\ref{fig:attacks} which is the working concept of ARM \textit{TrustZone Security Technology}. It virtually segregates system resources into \textit{secure} and \textit{non-secure} world. Besides, there are 2-bit RRESP and BRESP signal to acknowledge read and write transfers. Their status (OKAY, EXOKAY, SLVERR, DECERR) informs the master whether the transfer is successful or completed with error~\cite{ARMAXI2017}. But, if they are exposed to insider attacks or \textit{Hardware Trojan} can lead to intensive \textit{denial-of-service}, \textit{slave impersonation} and wide range of man-in-the-middle attacks~\cite{Benhani2017}.

%%
%%
%\begin{figure}[!b]
%\centerline{\includegraphics[scale=0.60]{PolicyEngine/Figs/axi4}}
%\caption{ARM AMBA-AXI4 compliant master-slave communication interface signals.}
%\label{fig:AXI4-channel}
%\end{figure}
%%
%%
%%----------------------------------------------------------------------------------%%
%% 			MPSoC based embedded policy engine architecture
%%----------------------------------------------------------------------------------%%
\subsection{Security policy Engine (SPE)}
\label{subsec:SPE}
%%
%%
The concept of SPE has inspired by the fundamental concepts of access control list in computer file systems introduced decades ago~\cite{Sandhu1994}. It checks the issued AXI4 transactions, compares it against an approved list of master, and either grants or restrict access to a attached slave. Fig.~\ref{fig:platform} shows the distributed deployment of SPE to enforce resource specific security measures by active monitoring of communications between system-bus and the slave (memory, sensor, actuator etc.). It is composed of the following five hardware blocks
%an \textit{AXI4 sniffer block, Device table, Policy table, Decision block} and \textit{Engine configuration block}. These hardware components are 
as shown in Fig.~\ref{fig:SPE}.
%%
%%
\begin{figure}[!t]
\centerline{\includegraphics[scale=0.65]{PolicyEngine/Figs/attacks}}
\caption{Block diagram illustrating possible insider attacks in MPSoC system.}
\label{fig:attacks}
\end{figure}
%%
%%
%%
%%
\begin{figure}[!b]
\centerline{\includegraphics[scale=0.60]{PolicyEngine/Figs/tables}}
\caption{Block diagram of Security Policy Engine (SPE).}
\label{fig:SPE}
\end{figure}
%%
%%
%%----------------------------------------------------------------------------------%%
%% 			Hardware components of secure policy engine
%%----------------------------------------------------------------------------------%%
%%
%%
\subsubsection{Engine configuration block} 
It allows to program and configure the security parameters of the SPE via AXI4-Lite interface through a \textit{secure application} running on the RPU as shown in Fig.~\ref{fig:platform}. It facilitates dynamic changes and updating system-level security policies if compromised.

\subsubsection{AXI4-Sniffer} 
It monitors and maintains the mandatory handshake signals until the \textit{decision block} checks and grants access to the slave which ensures correct system communication bus operations. It receives transactions from the shared system communication bus and samples the \textit{master} and \textit{slave} addresses using AxADDR and forwards it to the \textit{policy table}. Though, this work uses AxUSER signal to uniquely identify master and slave devices and do not rely on the system generated identification tags (AxID, xID). It uses AxVALID signals to identify read and write transactions. Once sampled, the address is passed to the \textit{device table} as shown in Fig.~\ref{fig:SPE}. During this process, it maintains physical isolation between system-bus and slave by de-asserting AxVALID signals to slave and AxREADY control signals to the system-bus.

\subsubsection{Device table} 
It holds a list of \textit{trusted masters} to access the slave. Each \textit{trusted master} list entry has corresponding base-address of the \textit{Policy table} as shown in Fig.~\ref{fig:SPE}. Generally, the number of slaves within the system are limited. Therefore, it is more area efficient to realised it using distributed RAM (LUT) resources of FPGA. It allows to filter out the transactions issued by \textit{trusted} and \textit{un-trusted} masters which facilitates \textit{intrusion detection}. In case of intrusion or malicious activity can be passively curtailed or actively suppressed by reporting to initiate defined pro-active response by SRE.
 
\subsubsection{Policy table} 
It contains a list of fine-grained (slave register) security access policies assigned to each \textit{trusted} master. These policies can be simple as read and write permissions, or security tailored security attributes (AxPROT) or quality of service (AxQoS). It can be realised by block RAM (BRAM) in FPGA logic. It allows to detect and suppress fine-grained intrusion or malicious activity (explicit modification of security attributes) introduced by the \textit{Hardware Trojan} as illustrated in Fig.~\ref{fig:attacks}. It can also caused by the compromised \textit{trusted master} and is not detected during \textit{Device table} look-up. An additional benefit is flexibility to provision embedded devices by defining policies during the operational life cycle of the device independent of silicon manufacturer, third-party vendors and hardware designers.

\subsubsection{Decision block} 
It receives the policy from the \textit{Policy table}, compares the security attributes of issued transaction against the expected behaviour and generates a result as shown in Fig.~\ref{fig:SPE}. This result is passed back to \textit{AXI-Sniffer}, which either physically grant access or keep it blocked to the slave.

%%
%%
\begin{table*}[!t]
\centering
\caption{Synthesis results of proposed security policy engine (SPE) on Zynq-7000 and Zynq UltraScale+ MPSoC.}
\label{tab:SPE-results}
\begin{tabular}{|l||l|c|cccc|c|}
\hline
\textbf{MPSoC} 	& \textbf{FPGA fabric} & \textbf{Speed} & \multicolumn{4}{c|}{\textbf{Area}} & \textbf{Frequency} \\
\cline{4-7}
      			& \textbf{(technology)}	& \textbf{Grade} & \textbf{LUT} & \textbf{LUTRAM} & \textbf{FF} & \textbf{BRAM} & \textbf{(MHz)} \\
\hline
\hline
\textbf{Zynq-7000} 	& Kintex-7 (28nm) 	& -3 		 & 87   & 32 & 304 & 1 & 250 \\
\textbf{Zynq UltraScale+ EG} & Kintex UltraScale+ (16nm) & -3 & 55   & 32 & 235 & 1 & 333\\
\hline
\end{tabular}
\end{table*}
%%
%%

%%----------------------------------------------------------------------------------%%
%% 			AXI4 bus sanity checker architecture
%%----------------------------------------------------------------------------------%%
\subsection{AXI4-Bus sanity checker (SCK)}
\label{subsec:sanity}
%%
%%
It ensures the integrity of the response status issued by the slaves back to the host processor by deploying between the host and the interconnect as illustrated in Fig.~\ref{fig:attacks}. It can mitigate insider attacks launched by \textit{Hardware Trojan}~\cite{Benhani2017}. It is composed of a \textit{finite state machine} (FSM) and a 32-bit counter implemented as a timer which is configurable via AXI4-Lite interface by the RPU. It has a CONTROL and STATUS register that enable/disable system-bus sanity checking and maintains the system status reported by the SRE. In case of an attack, SLVERR or DECERR force FSM to DETECTION state and timer start to decrement from the set value at each clock cycle. If it time-out the FSM transit to ATTACK state and report it to SRE to take countermeasure actions. On the contrary, FSM returns back to NORMAL state once SLVERR/DECERR signal is de-assert by the slave.

%%----------------------------------------------------------------------------------%%
%% 							Security Response Engine
%%----------------------------------------------------------------------------------%%
\subsection{Security Response Engine (SRE)}
\label{subsec:SRE}
%%
%%
It manages and triggers the active responses against malicious activity or hardware attacks reported by the \textit{decision block}. It interrupts the \textit{secure code} running on the RPU and runs executes priority interrupt service routine that initiates the pro-active response enforced by ATE which are:
%%
%%
\begin{itemize}
	\item Erasure of secret keys stored in the device.
	\item Permanently disable the system cryptographic functions.
	\item Disabling system read-back interfaces.
	\item Secure system lock-down.
	\item System reset.
\end{itemize}
%%
%%
%%----------------------------------------------------------------------------------%%
%% 							Security Response Engine
%%----------------------------------------------------------------------------------%%
\subsection{Anti-tamper Engine (ATE)}
\label{subsec:ATE}
%%
%%
It enforces the active countermeasures initiated by the SRE as well as, passive anti-tamper countermeasures against physical attacks. It independently monitors device physical parameters (voltage, temperature, power), which if violated raises an alarm in the form of system level interrupt.

%%----------------------------------------------------------------------------------%%
%% 							Implementation Results
%%----------------------------------------------------------------------------------%%
\subsection{Area and timing results}
\label{subsec:impl-results}
%%
%%
The proposed security policy engine (SPE) and its hardware components presented in Section 4.2 were coded in Verilog HDL. The design was simulated and synthesised using Xilinx Vivado v2017.1 on the high-end chips of the Zynq-7000 and Zynq UltraScale+ MPSoC family. The area and timing results are reported in Table 2. The device table implemented using Distributed RAM utilises 32 LUTRAM, while the policy table used a BRAM. The design is compact and consumes less than 1\% of FPGA glue logic available on Zynq chips. The reported timing results shows that SPE can operate at maximum 250 MHz and 333 MHz on Kintex-7 and Kintex UltraScale+ chips. The reported timing is limited by the maximum possible speed of ARM AMBA-AXI4 bus on these chips [40], [41].

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> RelatedWork/RelatedWork2.tex <==
\section{Related-work}
\label{sec:related-work}
%%
%%
This section will survey security vulnerabilities and short-falls reported in open literature on embedded MPSoC architectures and their supported security features.

%%
%% Reported attacks against ARM TrustZone technology
%%
Chen~\etal exploited the secure area of the main processor to load a malicious application and gain access to the device's secret data, breaching the loading verification process used by ARM's TrustZone technology. The attacker exploited a lack of proper rollback protection within the device's \textit{secure boot} process, using an old key to load a malicious application that could run in the secure-world, providing access to the device's secret data~\cite{Chen2017}. Jacob~\etal also described an attack against the \textit{secure boot} mechanism on FPGA MPSoC, which is important for ensuring secure system start-up and building chain-of-trust in embedded devices~\cite{Jacob2017}. This attack allowed modification of the kernel boot parameters, to load an unauthorised kernel image from a remote server over the network instead of booting from the verified source. Mitigation of these attacks, by formulating a well-defined policy for distributing patches and updating configurations to revoke older software versions, across a wide range of devices, is difficult from a practical perspective. Lipp~\etal further attacked the ARM TrustZone security extension using side-channel analysis. By monitoring cache activity in the special area of the Android operating system, they were able to infer and extract details of the last running process~\cite{Lipp2015}. Mitigation of cache-based attacks could be through deployment of separate caches for each virtual context, or to clear the cache when switching from secure to the non-secure world. \\
%Frédéric Basse, a security engineer has launched attack against an Amlogic S905 processor that uses ARM TrustZone for DRM and other security features. He successfully managed to bypass secure boot and break the chain-of-trust deploying series of attacks
%%
%% Concept of Hardware firewall using security policies
%%
Cotret~\etal have proposed a \textit{hardware firewall} architecture to protect external and internal traffic in multiprocessor architectures and digital circuits implemented on the FPGA. Their solution serves as security bridge between the system resources (memory and peripherals) and the shared system communication bus, to monitor control activities. Their \textit{hardware firewall} enforce security policies which are programmable to meet the dynamic security requirements of different applications. Their proposed work reduces the performance penalty compared to encrypt-all approach, but still guarantees asset protection against unprotected code and data. However, this architecture is limited to the detection of attacks and does not effectively mitigate against detected attacks, apart from freezing the system communication bus~\cite{Cotret2016}.\\
%%
%% Security evaluation of FPGA MPSoC and AXI4 specific vulnerabilities
%%
Jacob~\etal presented a detailed study of available on-chip security mechanisms in FPGA MPSoC chips. Although the availability of reconfigurable logic (FPGA) on the same die can be used to open a door to \textit{hardware trojans}~\cite{Jacob2017HWTrojan}, they have proposed a concept of building AXI-wrapper for each hardware core, similar to that proposed by Cotret~\etal, that encapsulates the device assets. Following this work, Benhani~\etal has presented a security evaluation of the ARM TrustZone technology available on FPGA MPSoC. They have presented a number of possible hardware attack scenarios that can be caused due to presence of \textit{hardware trojans} residing within the reconfigurable logic (FPGA) of the MPSoC~\cite{Benhani2017}. These \textit{hardware trojans} can be introduced during chip manufacturing process or at different stages of the device life-cycle. They have demonstrated that it is possible to modify hardware security attributes in a MPSoC system, that uses ARM TrustZone technology, and propagate them to the host processor by targeting AMBA-AXI4 communication system bus. To mitigate these vulnerabilities, they have proposed dividing system into secure and non-secure sub-systems. However, this strategy is not viable for systems with mixed criticality~\cite{Tan2016},~\cite{Tan2017}.
%%-----------------------------------------------------------------------------------------------------
%%
%%-----------------------------------------------------------------------------------------------------
\subsection{Shortcomings of existing security approaches}
\label{subsec:shortcomings}
%%
%%
After reviewing current state-of-art FPGA-based hardware security architectures, methodologies and mechanisms to approach various hardware security problems that can be used to secure existing and next-generation embedded systems. There is a clear evidence that the existing approaches fall-short due to:
%%
%%
\begin{itemize}
\item Security of major security architecture rely on building and maintaining robust chain-of-trust to make an architecture intrinsically secure. The chain-of-trust is based on a nested series of assumptions and as vulnerable as its weakest link which once broken compromised the security of the whole system.
%even a single vulnerability can be exploited to break the chain-of-trust leading to compromised system.
\item Lack of security aware design and development practises, embedded security standards, development of inconsistent and vulnerable software applications and complex hardware software co-design practises are key that give rise to vulnerabilities during life-cycle of the device. These vulnerabilities have extensively exploited by the attackers targeting hardware, software and their protocol stack boundaries to launch the insider and outsider attacks.
\item Unavailability of software independent run-time security mechanisms that can detect, curtail and secure system assets in hardware if the existing system security mechanisms are compromised. It includes systems with compromised chain-of-trust.   
\item Lack of hardware security standard which vendors can use to evaluate security of developed hardware and software components before integrating them into the system to ensure secure product development life-cycle.
\end{itemize}
%%
%%
%\blue{For silicon and IP manufacturers business point-of-view, embedded device security could be a feature which can be enabled and disabled, or even provides multiple level of security protections (basic protection, tamper detection, anti-tamper response etc.) depending on the desired application uses-case, level of security, conformance to the standard etc. To meet versatile IoT application requirements, it can be flexible/on-demand hierarchical segregation of system resources into multiple secure islands that can only exchange data within their designated secure island.}

